Processing SPARQL Queries Over Distributed RDF Graphs

We propose techniques for processing SPARQL queries over a large RDF graph in a distributed environment. We adopt a "partial evaluation and assembly" framework. Answering a SPARQL query Q is equivalent to finding subgraph matches of the query graph Q over RDF graph G. Based on properties of subgraph matching over a distributed graph, we introduce local partial match as partial answers in each fragment of RDF graph G. For assembly, we propose two methods: centralized and distributed assembly. We analyze our algorithms from both theoretically and experimentally. Extensive experiments over both real and benchmark RDF repositories of billions of triples confirm that our method is superior to the state-of-the-art methods in both the system's performance and scalability.

==> framework.tex <==
%!TEX root =  distributedgStore.tex
\section{Framework and Intuition}
\label{sec:framework}

As mentioned in the Introduction, our approach involves finding both inner matches within a fragment and crossing matches across fragments. Inner matches can be found locally at each site using existing centralized techniques (e.g., gStore \cite{Zou:2013fk} that we use in our tests). Therefore, we focus our discussion on computing crossing matches.


We propose a \emph{partial evaluation and assembly} \cite{DBLP:journals/csur/Jones96} framework to answer SPARQL queries over a distributed RDF graph $G$. In a distributed graph $G$, each site $S_i$ treats fragment $F_i$ as the known input $s$ and other fragments as yet unavailable input $d$ \cite{fan:reachability}.


Consider the case in Example \ref{example:crossingmatch}. The crossing match $M$ overlaps with two fragments $F_1$ and $F_2$.
If we can find the overlapping parts between $M$ and $F_1$, and $M$ and $F_2$, we can assemble them to form a crossing match. For example, the subgraph induced by vertices 014, 007, 001 and 002 is an overlapping part between $M$ and $F_1$. Similarly, we can also find the overlapping part between $M$ and $F_2$. We assemble them based on the common edge $\overrightarrow{002,001}$ to form a crossing match, as shown in Figure \ref{fig:assembly}.

\begin{figure}[h]
\begin{center}
    \includegraphics[scale=0.25]{pics/zlpartialmatch123.pdf}
       \vspace{-0.1in}
   \caption{Assemble Local Partial Matches}
   \label{fig:assembly}
   \vspace{-0.2in}
\end{center}
\end{figure}




In our execution model, each site $S_i$ ($i=1,...,k$) receives the full query graph $Q$. In the partial evaluation stage, at each site $S_i$, we find all \emph{local partial matches} (Definition  \ref{def:localmaximal}) of $Q$ in $F_i$. We prove that an overlapping part between any crossing match and fragment $F_i$ must be a local partial match in $F_i$ (see Theorem \ref{theorem:overlapping}).


In the assembly stage, these local partial matches are assembled to form crossing matches. In this paper, we consider two assembly strategies: centralized and distributed (or parallel). In centralized, all local partial matches are sent to a single site for the assembly. In distributed/parallel, local partial matches are combined at a number of sites in parallel. The details are in Section \ref{sec:assembling}.


Three are three steps in our method.

\textbf{Step 1} (\emph{Initialization}): A SPARQL query $Q$ is input and sent to each site $S_i$, $i=1,...,k$.


\textbf{Step 2} (\emph{Partial Evaluation}): Each site $S_i$ finds inner matches and \emph{local partial matches} of $Q$ in fragment $F_i$. This step is executed in  parallel at each site (Section \ref{sec:partialcomputing}).

\textbf{Step 3} (\emph{Assembly}): Finally, we assemble all local partial matches to form complete crossing matches. The system can use the centralized (Section \ref{sec:centralized}) or the the distributed assembly approach (Section \ref{sec:distributed}) to find crossing matches.

